Characterization of a Meso-Scale Wearable Robot for Bathing Assistance

Robotic bathing assistance has long been considered an important and practical task in healthcare. Yet, achieving flexible and efficient cleaning tasks on the human body is challenging, since washing the body involves direct human-robot physical contact and simple, safe, and effective devices are needed for bathing and hygiene. In this paper, we present a meso-scale wearable robot that can locomote along the human body to provide bathing and skin care assistance. We evaluated the cleaning performance of the robot system under different scenarios. The experiments on the pipe show that the robot can achieve cleaning percentage over 92% with two types of stretchable fabrics. The robot removed most of the debris with average values of 94% on a human arm and 93% on a manikin torso. The results demonstrate that the robot exhibits high performance in cleaning tasks.

==> coverletter.tex <==
Dear Dr. Asfour,

I am enclosing a manuscript entitled "Characterization of a Meso-Scale Wearable Robot for Bathing Assistance" for consideration for publication as a journal article in IEEE Robotics and Automation Letters. In our paper, we present a mobile robot that that can locomote along the human body to provide bathing and skin care assistance. The characterization experiments showed that our robot removed over $91$\% of the debris on cylindirical objects, human arm, and manikin torso. 

With this submission, I, as corresponding author on behalf of all the authors, confirm that this manuscript represents original research of which all authors played a significant role. This manuscript has not been published elsewhere, accepted for publication elsewhere, or under editorial review for publication elsewhere.

Thank you for your time and consideration.

Warm regards,
Fukang Liu
